Flexible Load Balancing with Multi-dimensional State-space Collapse: Throughput and Heavy-traffic Delay Optimality

Heavy traffic analysis for load balancing policies has relied heavily on the condition of state-space collapse onto a single-dimensional line in previous works. In this paper, via Lyapunov-drift analysis, we rigorously prove that even under a multi-dimensional state-space collapse, steady-state heavy-traffic delay optimality can still be achieved for a general load balancing system. This result directly implies that achieving steady-state heavy-traffic delay optimality simply requires that no server is idling while others are busy at heavy loads, thus complementing and extending the result obtained by diffusion approximations. Further, we explore the greater flexibility provided by allowing a multi-dimensional state-space collapse in designing new load balancing policies that are both throughput optimal and heavy-traffic delay optimal in steady state. This is achieved by overcoming various technical challenges, and the methods used in this paper could be of independent interest.

==> proof_general.tex <==
% !TEX root = ./sig2018_winter.tex
% \subsection{Proof of Proposition \ref{prop:prop_3}}
% \label{sec:proof_prop_3}
% \begin{proof}
% 	It follows from Claim \ref{claim_1} and the proof of Theorem \ref{thm:theorem_1} that the key for heavy-traffic delay optimality is the term $\mathcal{T}^{(\epsilon)}$. Instead of using Cauchy-Schwartz inequality, we apply H\"older inequality in Eq. \eqref{eq:upper_T} to obtain a tighter bound of $\mathcal{T}^{(\epsilon)}$ as follows. 
% 	\begin{align}
% 	\label{eq:upper_T_general}
% 		\mathcal{T}^{(\epsilon)} & \le \ex{\inner{\overline{\UU}}{-N_1\overline{\Q}^+_{\perp}}}\nonumber\\
% 		& \lep{a} \frac{N}{\alpha^{(\epsilon)}} { \left(\ex{\norm{\overline{\UU}}^{r'}_{r'} } \right)^{\frac{1}{r'}}  \left(\ex{\norm{\overline{\Q}^+_{\perp}}^r_r} \right)^{\frac{1}{r}}}.\nonumber\\
% 		& \lep{b} \frac{N}{\alpha^{(\epsilon)}}  \left(c_{r'} \epsilon \right)^{\frac{1}{r'}} \left(\ex{\norm{\overline{\Q}^+_{\perp}}^r_2} \right)^{\frac{1}{r}}.\nonumber\\
% 		& \lep{c}\frac{N}{\alpha^{(\epsilon)}}  \left(c_{r'} \epsilon \right)^{\frac{1}{r'}} \left(\ex{\norm{\overline{\Q}_{\perp}}^r_2} \right)^{\frac{1}{r}}.
% 	\end{align}
% 	where (a) follows from H\"older inequality for random vectors, and $r, r'\in (1,\infty)$ satisfy $1/r + 1/r' = 1$; (b) comes from Lemma \ref{lem:unused_service} and the fact that if $0<r_1 < r_2$, then $\norm{\mathbf{x}}_{r_2} \le \norm{\mathbf{x}}_{r_1}$ holds for any vector $\mathbf{x}$; (c) is true since the distribution of $\Q(t+1)$ and $\Q(t)$ are the same in steady-state.

% 	Thus, in order to prove the result in Proposition \ref{prop:prop_3}, we are left to characterize the moment of $\overline{\Q}_{\perp}$ in terms of the parameter $\delta^{(\epsilon)}$. First, combining Eq. \eqref{eq:drift_in_delta} and Claim \ref{claim_3}, yields
% 	\begin{equation*}
% 		\begin{split}
% 			&\ex{\Delta V_\perp(\Q) \mid \Q(t) = \Q }\\
% 		   \le & \frac{1}{2\norm{\Qc(t)}} \ex{\left(2\inner{\Qc(t)}{\A(t) - \s(t)} + L\right) \mid \Q(t) = \Q}\\
% 		   \le & -\frac{\mu_{\Sigma}\delta}{4N}  + \frac{L}{2\norm{\Qc(t)}}\\
% 		   \le & -\frac{\mu_{\Sigma}\delta}{8N} \text{ for all } \Q \text{ such that } \norm{\Qc} \ge \frac{4NL}{\mu_{\Sigma}\delta}.
% 		\end{split}
% 	\end{equation*}
% 	Thus the condition (C1) in Lemma \ref{lem:basis} is valid with $\eta = \frac{\mu_{\Sigma}\delta}{8N}$ and $\kappa = \frac{4NL}{\mu_{\Sigma}\delta}$. Also, from Eq. \eqref{eq:boundedQc}, we have the condition (C2) is valid with $D = \sqrt{N} \max(A_{\max},S_{\max})$. Then from Eq. \eqref{eq:upper_siva} in Lemma \ref{lem:basis}, we get for $r = 1,2,\ldots,$
% 	  \begin{align}
% 	  \label{eq:moment_in_delta}
% 	        	\ex{\norm{\overline{\Q}_{\perp}}^r_2} &\le (2\kappa)^r + (4D)^r\left(\frac{D+\eta}{\eta} \right)^r r!\nonumber\\
% 	        	&\le \frac{1}{\delta^r}K_r^r
% 	  \end{align}
% 	  where $K_r \triangleq \left[ \left(\frac{8NL}{\mu_{\Sigma}}\right)^r + r! \left(\frac{32D^2N + 4D\mu_{\Sigma}}{\mu_{\Sigma}}\right)^r \right]^{\frac{1}{r}}$, which is independent of $\epsilon$. Now, substituting Eq. \eqref{eq:moment_in_delta} into Eq. \eqref{eq:upper_T_general}, yields
% 	  \begin{align*}
% 	  	\mathcal{T}^{(\epsilon)} \le F_r\frac{\epsilon^{(1-1/r)}}{\alpha^{(\epsilon)}\delta^{(\epsilon)}}
% 	  \end{align*}
% 	  where $F_r \triangleq NK_r(S_{\max})^{(1/r^2 - 1/r)}$, which is independent of $\epsilon$. Since $\alpha^{(\epsilon)}\delta^{(\epsilon)} = \Omega(\epsilon^{\beta})$ and $\beta \in [0,1)$, there exists a positive $\beta'$ such that 
% 	  \begin{align*}
% 	  	\mathcal{T}^{(\epsilon)} = O(\epsilon^{\beta'}),
% 	  \end{align*}
% 	  when $r > 1/(1-\beta)$. This directly implies that $\lim_{\epsilon \to 0}\mathcal{T}^{(\epsilon)} = 0$. Thus from Claim \ref{claim_1}, the given policy is heavy-traffic delay optimal.

% \end{proof}
